Pseudo-Boolean d-DNNF Compilation for Expressive Feature Modeling Constructs

Configurable systems typically consist of reusable assets that have dependencies between each other. To specify such dependencies, feature models are commonly used. As feature models in practice are often complex, automated reasoning is typically employed to analyze the dependencies. Here, the de facto standard is translating the feature model to conjunctive normal form (CNF) to enable employing off-the-shelf tools, such as SAT or #SAT solvers. However, modern feature-modeling dialects often contain constructs, such as cardinality constraints, that are ill-suited for conversion to CNF. This mismatch between the input of reasoning engines and the available feature-modeling dialects limits the applicability of the more expressive constructs. In this work, we shorten this gap between expressive constructs and scalable automated reasoning. Our contribution is twofold: First, we provide a pseudo-Boolean encoding for feature models, which facilitates smaller representations of commonly employed constructs compared to Boolean encoding. Second, we propose a novel method to compile pseudo-Boolean formulas to Boolean d-DNNF. With the compiled d-DNNFs, we can resort to a plethora of efficient analyses already used in feature modeling. Our empirical evaluation shows that our proposal substantially outperforms the state-of-the-art based on CNF inputs for expressive constructs. For every considered dataset representing different feature models and feature-modeling constructs, the feature models can be significantly faster translated to pseudo-Boolean than to CNF. Overall, deriving d-DNNFs from a feature model with the targeted expressive constraints can be substantially accelerated using our pseudo-Boolean approach. Furthermore, our approach is competitive on feature models with only basic constructs.

==> latexutils/constants/bib.tex <==
\newcommand{\bibtags}{\string~/git/latex/BibTags}


\newcommand{\bibacm}{
	\bibliographystyle{ACM-Reference-Format}
	\bibliography{/home/chico/git/latex/BibTags/MYabrv,/home/chico/git/latex/BibTags/literature-cleaned,/home/chico/git/latex/BibTags/toMergeEdited}
}

\newcommand{\bibacmshort}{
	\bibliographystyle{ACM-Reference-Format}
	\bibliography{/home/chico/git/latex/BibTags/MYshort,/home/chico/git/latex/BibTags/literature-cleaned,/home/chico/git/latex/BibTags/toMergeEdited}
}

==> latexutils/core/bool.tex <==
\newcommand{\ptrue}{\mbox{\textit{true}}}
\newcommand{\pfalse}{\mbox{\textit{false}}}
\newcommand{\pnull}{\mbox{\textit{null}}}
\newcommand{\pnot}{\neg}
\newcommand{\pand}{\wedge}
\newcommand{\por}{\vee}
\newcommand{\pxor}{\oplus\ }
\newcommand{\pequals}{\Leftrightarrow}
\newcommand{\pimplies}{\Rightarrow}
\newcommand{\pnimplies}{\nRightarrow}
\newcommand{\patmostone}{\mbox{\textit{atmost1}}}
\newcommand{\pchooseone}{\mbox{\textit{choose1}}}
\newcommand{\pbigand}{\bigwedge}
\newcommand{\pbigor}{\bigvee}
\newcommand{\pbigxor}{\bigoplus}
\newcommand{\ptaut}{\models}
\newcommand{\pntaut}{\not\models}

\newcommand{\pSAT}{SAT}
\newcommand{\pSharpSAT}{\#SAT}

==> latexutils/core/code.tex <==
\newcommand{\code}[1]{\texttt{#1}}
\newenvironment{codediffsnippet}{\center\small\BVerbatim[commandchars=\\\{\}]}{\endBVerbatim\endcenter}

==> latexutils/core/lst.tex <==
%%% \usepackage{listings}
\lstset{escapeinside={<@}{@>}}

==> latexutils/core/math.tex <==
%%% \usepackage{amsmath}
%%% \usepackage{amsthm}

\DeclareMathOperator{\naturalNumbers}{\mathbb{N}}
% \DeclareMathOperator{\powerset}{\mathcal{P}}
\DeclareMathOperator{\mapstoSpace}{\rightarrow}
\DeclareMathOperator{\setunion}{\cup}
\DeclareMathOperator{\setcut}{\cap}
\DeclareMathOperator{\bigsetunion}{\bigcup}
\DeclareMathOperator{\bigsetcut}{\bigcap}
\DeclareMathOperator{\setdisjunctunion}{\dot\cup}

\providecommand{\myqed}{\hfill\ensuremath{\square}}

==> latexutils/core/misc.tex <==
\newcommand{\myvautoref}[1]{\autoref{#1} on Page \pageref{#1}}

==> latexutils/core/tabular.tex <==
\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
%%% args are rotation in degrees and content
\newcommand{\dTableHeader}[2]{\rotatebox[origin=c]{#1}{#2}}
%%% args are content and width
\newcommand*{\dPatternTableHeader}[2]{\dTableHeader{80}{\parbox{#2}{#1}}}

==> latexutils/languages/lst.tex <==
\usepackage{listings}

\definecolor{eclipseStrings}{RGB}{42,0.0,255}
\definecolor{eclipseKeywords}{RGB}{127,0,85}
\colorlet{numb}{magenta!60!black}

\lstdefinelanguage{json}{
    basicstyle=\normalfont\ttfamily\footnotesize,
    commentstyle=\color{eclipseStrings}, % style of comment
    stringstyle=\color{eclipseKeywords}, % style of strings
    numbers=left,
    numberstyle=\scriptsize,
    xleftmargin=0.6cm,
    stepnumber=1,
    numbersep=8pt,
    showstringspaces=false,
    breaklines=true,
    string=[s]{"}{"},
    comment=[l]{:\ "},
    morecomment=[l]{:"},
    tabsize=4,
    literate=
        *{0}{{{\color{numb}0}}}{1}
         {1}{{{\color{numb}1}}}{1}
         {2}{{{\color{numb}2}}}{1}
         {3}{{{\color{numb}3}}}{1}
         {4}{{{\color{numb}4}}}{1}
         {5}{{{\color{numb}5}}}{1}
         {6}{{{\color{numb}6}}}{1}
         {7}{{{\color{numb}7}}}{1}
         {8}{{{\color{numb}8}}}{1}
         {9}{{{\color{numb}9}}}{1}
}

\lstdefinelanguage{uvlsimple}{
	keywords = {alternative,or,optional,mandatory,features,constraints,include},
    % otherkeywords={=>,|,&},
	morecomment=[l]{//},
	commentstyle=\itshape\color{purple!40!black},
    keywordstyle=\ttfamily\color{eclipseKeywords},
    tabsize=4,
    columns=fullflexible
}

\lstdefinelanguage{uvlfull}{
	keywords = {alternative,or,optional,mandatory,features,constraints, cardinality, Real, Boolean, Integer, String, imports, as,include},
    otherkeywords = {|,&,[,], ==, \{,\}, =>, <},
	morecomment=[l]{//},
	commentstyle=\itshape\color{purple!40!black},
    keywordstyle=\ttfamily\color{eclipseKeywords},
    tabsize=4,
    columns=fullflexible
}


\lstdefinelanguage{dimacs}{
    keywords = {p,cnf,c},
    keywordstyle=\ttfamily\color{eclipseKeywords},
    columns=fullflexible,
    tabsize=4
}


==> latexutils/misc/algpseudocodeutils.tex <==
%%% \usepackage{algpseudocode}

%%% Define "for each" operator
\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

%%% Define "Assert" operator
\algnewcommand\algorithmicassert{\textbf{Assert}}
\algnewcommand\Assert[1]{\State \algorithmicassert{} #1}%

%%% Multiline comment
%%% #1: Optional argument. Number between 0 and 1 that describes the relative width of the comment in the algorithm environment. Defaults to 0.3.
%%% #2: Mandatory argument. The text that should be inside the comment.
\newcommand{\MultLineComment}[2][0.3]{\Comment{\parbox[t]{#1 \linewidth}{#2}}}

==> latexutils/misc/commandutils.tex <==
%%% Takes the name of a macro (first argument) and defines it with the given body (second argument).
\newcommand{\defineCommandByName}[2]{\expandafter\newcommand\csname #1\endcsname{#2}}

%%% Takes the name of a macro and runs the macro with that name without arguments.
%%% Make sure that the macro with the given name does not take any arguments.
%%% For example \runCommandByName{dots} will evaluate to \dots.
\newcommand{\runCommandByName}[1]{\csname #1\endcsname}

==> latexutils/misc/makeNameMacro.tex <==
%%% Depends on "misc/commandutils.tex"

%%% Given a command whose value represents a name, creates a new macro that represents the plural of that name.
%%% For example, the following:
%%%   \newcommand{\myFavouriteBread}{toast}
%%%   \makePluralMacro{myFavouriteBread}
%%% will create a new macro \toastpl that will evaluate to toasts.
%%% As an optional argument one may pass an alternative ending replacing "s".
%%% For instance, the plural of patch should be patches so you should use
%%%   \makePluralMacro[es]{patch}
\newcommand{\makePluralMacro}[2][s]{\expandafter\newcommand\csname #2pl\endcsname{\runCommandByName{#2}#1}}

==> latexutils/misc/names.tex <==
\newcommand{\tubs}{TU\allowbreak{} Braunschweig}

==> latexutils/misc/researchquestions.tex <==
%%% Depends on "misc/commandutils.tex"

%%% Utility methods to deal with research questions as named variables (and not with numbers)
%%% This hopefully helps to avoid ambiguity and confusion, and to allow secure renaming of research question numbers.

%%% internal counter to keep track of how many RQs are defined
\newcounter{rqcounter}
\setcounter{rqcounter}{1}

%%% With \defineRQ you can define your research question by providing
%%% - an identifier you want to use as the first argument
%%% - the question as text as the second argument
%%% The order in which you define your research questions matters as it defines their numbers.
%%% For example:
%%%     \defineRQ{SkyBlue}{Why is the sky blue?}
%%%     \defineRQ{EarthRound}{Why is the earth round?}
%%% will make SkyBlue be your first research question and EarthRound your second.
\newcommand{\defineRQ}[2]
{
	\newcounter{numOfRQ#1}
	\setcounter{numOfRQ#1}{\value{rqcounter}}
	\defineCommandByName{rqValue#1}{#2}
	\refstepcounter{rqcounter}
}

%%% With \refRQ you can reference a research question in your text.
%%% The argument to pass is the identifier of the research question you want to reference.
%%% For example:
%%%     We investigate \refRQ{SkyBlue} and \refRQ{EarthRound}.
%%% yields
%%%     We investigate RQ1 and RQ2.
%%% depending on the order you defined the research questions with \defineRQ.
\newcommand{\refRQ}[1]
{RQ\arabic{numOfRQ#1}}

%%% Gives the total amount of research questions you have.
\newcommand{\refNumRQs}[0]
{\the\numexpr\value{rqcounter}-1\relax}

%%% With \printRQ you can print the research question in your text.
%%% The argument to pass is the identifier of the research question you want to show.
%%% For example:
%%%     Our main questions is: \printRQ{SkyBlue}
%%% yields
%%%     Our main questions is: Why is the sky blue?
\newcommand{\printRQ}[1]
{\runCommandByName{rqValue#1}}

%%% \showRQInDescription is a shortcut to introduce your research questions in a desription environment.
%%% Example usage:
%%% \begin{description}
%%%     \showRQInDescription{SkyBlue}
%%%     \showRQInDescription{EarthRound}
%%% \end{description}
\newcommand{\showRQInDescription}[1]
{\item[\refRQ{#1}] \printRQ{#1}}


==> latexutils/misc/showfont.tex <==
%%% Print some information on the used font to your current document. I couldn't turn this into a command yet (got errors then), so \input this file somewhere in your document (between \begin{document} and \end{document}).

\makeatletter
encoding: \f@encoding{},
family: \f@family{},
series: \f@series{},
shape: \f@shape{},
size: \f@size{}
\makeatother

==> latexutils/misc/textbox.tex <==
\NewEnviron{textbox}{
	\begin{center}
		\setlength\fboxsep{0.5em}
		\fbox{
			\parbox{0.8\linewidth}{
				\BODY{}
			}
		}
	\end{center}
}

==> latexutils/misc/theorems.tex <==
\newtheorem{theorem}{Theorem}
\theoremstyle{definition}
\newtheorem{definition}{Definition}

==> latexutils/template/acm.tex <==
\newenvironment{myDescription}{\begin{description}}{\end{description}}

==> latexutils/template/ieee.tex <==
\newenvironment{myDescription}
{\LaTeXdescription}
{\endLaTeXdescription}

\theoremstyle{definition}
\newtheorem{definition}{Definition}

==> latexutils/variantsync/names.tex <==
\newcommand{\cloneandown}{clone-and-own}
\newcommand{\Cloneandown}{Clone-and-own}
\newcommand{\CloneandOwn}{Clone-and-Own}

% haha
\newcommand{\clownandown}{\cloneandown{}}
\newcommand{\Clownandown}{\Cloneandown{}}
\newcommand{\ClownAndOwn}{\CloneandOwn{}}

\newcommand{\variantsync}{\emph{VariantSync}}

==> latexutils/visualization/featuremodel.tex <==
%---required packages & variable definitions------------------------------------
\usepackage{forest}
\usepackage{xcolor}
\usetikzlibrary{angles}
\definecolor{drawColor}{RGB}{128 128 128}
\newcommand{\circleSize}{0.2em}
\newcommand{\angleSize}{0.8em}
%-------------------------------------------------------------------------------
%---Define the style of the tree------------------------------------------------
\forestset{
	/tikz/mandatory/.style={
		circle,fill=drawColor,
		draw=drawColor,
		inner sep=\circleSize
	},
	/tikz/optional/.style={
		circle,
		fill=white,
		draw=drawColor,
		inner sep=\circleSize
	},
	featureDiagram/.style={
		for tree={
			font=\footnotesize,
			text depth = 0,
			parent anchor = south,
			child anchor = north,
			draw = drawColor,
			edge = {draw=drawColor},
		}
	},
	/tikz/abstract/.style={
		fill = blue!85!cyan!5,
		draw = drawColor
	},
	/tikz/concrete/.style={
		fill = blue!85!cyan!20,
		draw = drawColor
	},
	mandatory/.style={
		edge label={node [mandatory] {} }
	},
	optional/.style={
		edge label={node [optional] {} }
	},
	or/.style={
		tikz+={
			\path (.parent) coordinate (A) -- (!u.children) coordinate (B) -- (!ul.parent) coordinate (C) pic[fill=drawColor, angle radius=\angleSize]{angle};
		}	
	},
	/tikz/or/.style={
	},
	alternative/.style={
		tikz+={
			\path (.parent) coordinate (A) -- (!u.children) coordinate (B) -- (!ul.parent) coordinate (C) pic[draw=drawColor, angle radius=\angleSize]{angle};
		}	
	},
	/tikz/alternative/.style={
	},
	/tikz/placeholder/.style={
	},
	collapsed/.style={
		rounded corners,
		no edge,
		for tree={
			fill opacity=0,
			draw opacity=0,
			l = 0em,
		}
	},
	/tikz/hiddenNodes/.style={
		midway,
		rounded corners,
		draw=drawColor,
		fill=white,
		minimum size = 1.2em,
		minimum width = 0.8em,
		scale=0.9
	},
}
%-------------------------------------------------------------------------------

% Example
% \begin{figure}
% 	\begin{forest}
% 		featureDiagram
% 		[Vending Machine,concrete[Transport,concrete,mandatory[Drop,concrete,alternative][Elevator,concrete]][Items,concrete,mandatory[Ice Cream,concrete,or][Chocolate,concrete][Drinks,concrete]][Cooling,concrete,optional]]
% 		\matrix [anchor=north west] at (current bounding box.north east) {
% 			\node [placeholder] {}; \\
% 		};
% 		\matrix [draw=drawColor,anchor=north west] at (current bounding box.north east) {
% 			\node [label=center:\underline{Legend:}] {};        \\
% 			\node [concrete,label=right:Feature] {};              \\
% 			\node [mandatory,label=right:Mandatory] {};           \\
% 			\node [optional,label=right:Optional] {};             \\
% 			\filldraw[drawColor] (0.1,0) - +(-0,-0.2) - +(0.2,-0.2)- +(0.1,0);
% 			\draw[drawColor] (0.1,0) -- +(-0.2, -0.4);
% 			\draw[drawColor] (0.1,0) -- +(0.2,-0.4);
% 			\fill[drawColor] (0,-0.2) arc (240:300:0.2);
% 			\node [or,label=right:Or Group] {};                   \\			
% 			\draw[drawColor] (0.1,0) -- +(-0.2, -0.4);
% 			\draw[drawColor] (0.1,0) -- +(0.2,-0.4);
% 			\draw[drawColor] (0,-0.2) arc (240:300:0.2);
% 			\node [alternative,label=right:Alternative Group] {}; \\};
% 		\matrix [anchor=north, align=center] at (0,-2) {
% 			\node {Drop $\Rightarrow \neg$ Drinks $\land$ $\neg$ Ice Cream}; \\
% 			\node {(Ice Cream $\vee$ Lemonade) $\Rightarrow$ Cooling};\\};
% 	\end{forest}
% 	\caption{Feature Model Example}
% 	\label{fig:motivation:pc}
% \end{figure}
